Truncated proposals for scalable and hassle-free simulation-based inference

Simulation-based inference (SBI) solves statistical inverse problems by repeatedly running a stochastic simulator and inferring posterior distributions from model-simulations. To improve simulation efficiency, several inference methods take a sequential approach and iteratively adapt the proposal distributions from which model simulations are generated. However, many of these sequential methods are difficult to use in practice, both because the resulting optimisation problems can be challenging and efficient diagnostic tools are lacking. To overcome these issues, we present Truncated Sequential Neural Posterior Estimation (TSNPE). TSNPE performs sequential inference with truncated proposals, sidestepping the optimisation issues of alternative approaches. In addition, TSNPE allows to efficiently perform coverage tests that can scale to complex models with many parameters. We demonstrate that TSNPE performs on par with previous methods on established benchmark tasks. We then apply TSNPE to two challenging problems from neuroscience and show that TSNPE can successfully obtain the posterior distributions, whereas previous methods fail. Overall, our results demonstrate that TSNPE is an efficient, accurate, and robust inference method that can scale to challenging scientific models.

==> equations.tex <==
@Jakob @Pedro: Please ignore this section, it is only for screenshotting equations for use in inkscape.

\begin{equation*}
    \min_{\bphi} \mathcal{L} = \min_{\bphi}\EX_{\btheta \sim \tilde{p}(\btheta)}\EX_{\bx \sim p(\bx|\btheta)}[-\log q_{\bphi}(\btheta|\bx)]
\end{equation*}

\begin{equation*}
    \btheta \sim p(\btheta)
\end{equation*}

\begin{equation*}
    \bx \sim p(\bx | \btheta)
\end{equation*}

\begin{equation*}
    q_{\phi}(\btheta | \bx_o)
\end{equation*}

\begin{equation*}
    \btheta
\end{equation*}

\begin{equation*}
    \bx
\end{equation*}

\begin{equation*}
    \min_{\bphi} \EX[-\log q_{\bphi}(\btheta|\bx)]
\end{equation*}

\begin{equation*}
    \mathcal{L} = \EX[-\log q_{\bphi}(\btheta|\bx)]
\end{equation*}

\begin{equation*}
    \mathrm{min}_{\bphi} \EX[-\log q_{\bphi}(\btheta|\bx)]
\end{equation*}

\begin{equation*}
    \tilde{p}(\btheta) \propto p(\btheta) \cdot \mathds{1}_{\btheta \in \text{supp}(p(\btheta | \bx))}
\end{equation*}

\begin{equation*}
    \btheta
\end{equation*}

\begin{equation*}
    \log(p(\btheta | \bx))
\end{equation*}


==> figures/fig3.tex <==
\begin{figure}[ht!]
\ifdefined\NOFIGS
    [FIGURE SKIPPED]
    [Comment out line 3 of main.tex to include]
\else
    \includegraphics[width=\linewidth]{./figures/fig3.png}
\fi
\caption{
%
{\bf Demonstration on two-moons task.}
%
The method starts by sampling from the prior, running the simulator, and training a neural density estimator with maximum likelihood to approximate the posterior. In subsequent rounds, parameters are sampled from the prior, but rejected if they lie outside of the support of the approximate posterior. With these proposals, the neural density estimator can be trained with maximum likelihood in all rounds.
}

\label{fig:fig3}
\end{figure}
